CarFi: Rider Localization Using Wi-Fi CSI

With the rise of hailing services, people are increasingly relying on shared mobility (e.g., Uber, Lyft) drivers to pick up for transportation. However, such drivers and riders have difficulties finding each other in urban areas as GPS signals get blocked by skyscrapers, in crowded environments (e.g., in stadiums, airports, and bars), at night, and in bad weather. It wastes their time, creates a bad user experience, and causes more CO2 emissions due to idle driving. In this work, we explore the potential of Wi-Fi to help drivers to determine the street side of the riders. Our proposed system is called CarFi that uses Wi-Fi CSI from two antennas placed inside a moving vehicle and a data-driven technique to determine the street side of the rider. By collecting real-world data in realistic and challenging settings by blocking the signal with other people and other parked cars, we see that CarFi is 95.44% accurate in rider-side determination in both line of sight (LoS) and non-line of sight (nLoS) conditions, and can be run on an embedded GPU in real-time.

==> tex/2.usage.tex <==

\section{Usage}


% how the passenger and driver are interacting with each other
We describe a real-world usage scenario of \CF in this chapter. When a passenger wants to travel to a specific location, he or she uses the ride-hailing app on the phone to book the trip. The server processes the request and finds the driver. The locations of the vehicle and the passenger are determined by their respective location providers, such as GPS on the phone. Once the trip is confirmed, the driver heads toward the passenger's location. As the driver arrives within a certain distance from the passenger based on the location data, the passenger's phone will transmit the WiFi packets at a higher packet rate as the ride-hailing app controls it. Meanwhile, the dashcam starts listening for WiFi packets containing the phone's MAC address. When \CF system receives the WiFi packets, it extracts the CSI information and calculates the features. Then it estimates where the passenger is, and the driver can proceed to the correct location. If the driver can only park the vehicle at specific parking spots safely, the relative location can also guide the passenger toward the vehicle.

==> tex/3.background.tex <==

\section{Background}

\subsection{Angle of Arrival (AoA)}
\label{sec:background_aoa}


When antennas receive an RF signal, the signal is coming from a certain direction. The angle of Arrival (AoA) is used to describe this direction. How the AoA is normally defined is shown in Figure~\ref{fig:ant_aoa}. The circular dots represent the antennas. The dashed line is the coordinate system of the antenna array. The vertical dash line, which is perpendicular to the antenna array, is the boresight of this array. Boresight is the axis of maximum gain, and for most antennas, the boresight is also the axis of symmetry. Suppose the antennas shown in the figure are omnidirectional antennas. In that case, signals coming from either side and mirroring along the antenna array (i.e., top or bottom in the figure) will have the same AoA.


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{figs/ant_aoa.pdf}
    \caption[Angle of arrival of RF signals]{Angle of arrival of RF signals are measured as the angle between the signal and the boresight of the antenna array.}
    \label{fig:ant_aoa}
\end{figure}


To calculate the AoA, the time difference of arrival (TDOA) is usually utilized. As the distance traveled by the signal is different for each antenna, as shown in the figure, the time will also be different. However, as RF signals traveling at the same speed as light, the time difference is usually too small to be effectively measured by the hardware. As a result, the phase difference between the received signals is generally used to estimate the AoA.


\subsection{Received Signal Strength Indicator (RSSI)}

Received Signal Strength Indicator (RSSI) is a measurement of the power present in a received radio signal. RSSI is usually derived in the intermediate frequency (IF) stage before the IF amplifier and is a relative index. The 802.11 standards do not specify detailed rules regarding RSSI, and each manufacturer can define their own max value. There is no defined relationship between the RSSI value to the actual power level in milliwatts or decibels referenced on one milliwatt (dBm), and each vendor and manufacture can define their own accuracy, granularity, and range for the actual power. As a result, it is usually not accurate to compare RSSI between different chips, but a higher value with the same chip means a better signal. The RSSI value can also be used internally to determine when the network card is clear to send (CTS).

Different from RSSI, which measures the received power in preamble only, Received Channel Power Indicator (RCPI) is introduced to measure the received RF power in the selected channel for the received frame. It is also defined that the RCPI shall equal the received RF power within an accuracy of $\pm5$ dB (95\% confidence interval) within the specified dynamic range of the receiver. 

%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Channel State Information (CSI)}

With newer IEEE 802.11 standards support Multiple-Input and Multiple-Output (MIMO) to increase the performance and stability of the WiFi systems, WiFi chipsets measure the channel at the Orthogonal Frequency-Division Multiplexing (OFDM) subcarrier level. The result is reported in a standard Channel State Information (CSI) format, as shown in Table~\ref{tab:csi_format}. In this table, grouping means the method used to reduce the size of the CSI report by reporting a single value for each group of N adjacent subcarriers. Ns is the number of subcarriers reported. 

\begin{table*}[]
    \centering
    \caption[CSI carriers reported based on carrier grouping]{CSI carriers reported based on carrier grouping. \citep{IEEEwifistandard}}
    \begin{tabular}{c|c|c|c}
        \toprule
         BW  & Grouping & Ns & Carriers for which matrices are sent \\ \hline \hline
         \multirow{3}{*}[-0.5em]{20 MHz} & 1 & 56 & All data and pilot carriers: –28, –27,…–2, –1, 1, 2,…27, 28 \\ \cline{2-4}
         & 2 & 30 & \makecell{–28,–26,–24,–22,–20,–18,–16,–14,–12,–10,–8,–6,–4,–2,–1,\\1,3,5,7,9,11,13,15,17,19,21,23,25,27,28} \\ \cline{2-4}
         & 4 & 16 & –28,–24,–20,–16,–12,–8,–4,–1,1,5,9,13,17,21,25,28 \\ \cline{1-4}
         \multirow{3}{*}[-2em]{40 MHz} & 1 & 114 & All data and pilot carriers: –58, –57, …, –3, –2, 2, 3,…, 57, 58 \\ \cline{2-4}
         & 2 & 58 & \makecell{–58,–56,–54,–52,–50,–48,–46,–44,–42,–40,–38,–36,–34,–32,–30,\\ –28,–26,–24,–22,–20,–18,–16,–14,–12,–10,–8,–6,–4,–2, \\ 2,4,6,8,10,12,14,16,18,20,22,24,26,28, \\ 30,32,34,36,38,40,42,44,46,48,50,52,54,56,58} \\ \cline{2-4}
         & 4 & 30 & \makecell{–58,–54,–50,–46,–42,–38,–34,–30,–26,–22,–18,–14,–10,–6, –2,\\2,6,10,14,18,22,26,30,34,38,42,46,50,54,58} \\ \bottomrule
    \end{tabular}
    \label{tab:csi_format}
\end{table*}

As CSI measures the subcarrier level, the information recorded is much granular than RSSI. The properties of such channels are a description of the combined effect of the scattering, fading, and power decay between the transmitter and receiver. Each CSI entry represents the Channel Frequency Response (CFR):

\begin{equation}
    H(f;t) = \sum_n^N a_n(t)e^{-j2\pi f\tau_n(t)}
\end{equation}

where $a_i(t)$ is the amplitude attenuation factor, $\tau_i(t)$ is the propagation delay, and $f$ is the carrier frequency~\citep{tse2005fundamentals}. Since the signals between the transmitters and receivers are impacted by the environment and the displacement and movement of the antennas themselves, the CSI amplitude $|H|$ and phase $\angle H$ captures the wireless characteristics of the environment. 


Before the data symbols are transmitted, the transmitter will send Long Training Symbols (LTFs), containing pre-defined symbols for each subcarrier. For each subcarrier, the signal is modeled as $y=Hx + n$, where $y$ is the received signal, $x$ is the transmitted signal, and $n$ is the noise. $H$ is the CSI matrix, as shown before. With the received LTFs and the known pre-defined LTFs that are transmitted, the chipset can estimate the matrix $H$. As a result, the reported CSI values are not the most accurate as it is also affected by other factors within the chipset. In recent studies, researchers have found that CSI can be used for WiFi sensing, including but not limited to: angle of arrival estimation, human detection, breath detection, and etc.



\subsection{MUSIC and Variants}

For the angle of arrival (AoA) estimation, one classical method is the MUSIC algorithm~\citep{schmidt1986multiple}. If two antennas are separated $d$ apart, the additional phase shift introduced due to the distance is $-2\pi\times d\times\sin(\theta)\times f/c$, where $\theta$ is the AoA, $f$ is the signal frequency, and $c$ is the speed of light. The MUSIC algorithm works by estimating the steering matrix $A$ in: $X = AF$, where $X$ is the measurement matrix of the received signal, and $F$ is the matrix of complex attenuation. In a recent WiFi-based localization algorithm~\citep{kotaru2015spotfi}, the AoA of the direct path (which is relevant to the localization problem) is isolated by taking the eigenvector of the matrix, $XX^H$, for which, the eigenvalue is zero. The eigenvector goes through further processing to obtain the direct path.



